On the Time-Dependent Analysis of Gamow Decay

Gamow's approach to exponential decay of meta-stable particles via complex 'eigenvalues' (resonances) of a Hamiltonian is scrutinized. We explain the sense in which the non-square-integrable 'eigenfunctions' that belong to these resonances (Gamow functions) are relevant for the time-evolution of square-integrable wave functions. For concreteness we study a one dimensional square-well potential with a trapping region K and the evolution of wave functions, whose support is initially inside of K. It is shown that the sum over the first few time-evolved Gamow functions restricted to K yields an approximation for the evolution of these initial wave functions within the trapping region. The approximation is good for all times for which exponential decay prevails.

==> module5.tex <==
%\documentclass[a4paper,10pt]{amsbook}

%\usepackage[latin1]{inputenc}
%\usepackage[english]{babel}
%%\usepackage[pdftex]{hyperref}
%\usepackage{a4wide}
%\usepackage{amsmath,amssymb,amsthm}
%\usepackage{fancyhdr}
%\usepackage{srctex}
%%\hypersetup{colorlinks}

%\begin{document}
{\huge\textbf{Acknowledgment}}
\vspace{1cm}

First and foremost I would like to thank my mother Andrea~Grummt wholeheartedly.
Her steady encouragement and her boundless financial support made not only this
thesis possible, but it also allowed me to delve into physics in the first
place. And I am deeply thankful for that. In the same breath, I would like to
thank my father Rolf~Oppermann. I am indebted to him in many respects, but
especially for all the discussions about the things that became so important to
me. Both of you are the reason I am an independently thinking person today.

I also want to express my deep gratitude to my mentor Detlef~Dürr. He showed me
what it means to understand a thing and thereby he showed me the pleasure that
is connected with clear-cut understanding. I am looking forward to all the
discoveries, which are waiting for us.

In the last year, Martin~Kolb patiently answered numerous mathematical questions
of mine. He showed me the loopholes in my arguments and helped me getting to the
bottom of things. I want to thank him for that. And I want to thank Peter~Pickl
with whom I had numerous discussions on the subject of this thesis which were
invaluable for shaping my ideas. 

My grandparents Helmut and Hildegard Grummt as well as Arno and Walburga
Schultchen contributed to the success of this work, too. I want to thank them
for their steady support, which made more things possible for me than I probably
know.

Moreover, I would like to thank my friends Philipp~Reineck, Lukas~Ost and
Britta~Milde for proofreading my work on short notice.

Last but not least, special thanks go out to one very special person,
Carina~Pelzl. Over the last few years she was more than patient with me and my
dedication to physics. Your support means more to me than you can imagine.


%\bibliographystyle{plain}
%\bibliography{citations}
%\end{document}

